Exploring the Boundaries of On-Device Inference: When Tiny Falls Short, Go Hierarchical

On-device inference holds great potential for increased energy efficiency, responsiveness, and privacy in edge ML systems. However, due to less capable ML models that can be embedded in resource-limited devices, use cases are limited to simple inference tasks such as visual keyword spotting, gesture recognition, and predictive analytics. In this context, the Hierarchical Inference (HI) system has emerged as a promising solution that augments the capabilities of the local ML by offloading selected samples to an edge server or cloud for remote ML inference. Existing works demonstrate through simulation that HI improves accuracy. However, they do not account for the latency and energy consumption on the device, nor do they consider three key heterogeneous dimensions that characterize ML systems: hardware, network connectivity, and models. In contrast, this paper systematically compares the performance of HI with on-device inference based on measurements of accuracy, latency, and energy for running embedded ML models on five devices with different capabilities and three image classification datasets. For a given accuracy requirement, the HI systems we designed achieved up to 73% lower latency and up to 77% lower device energy consumption than an on-device inference system. The key to building an efficient HI system is the availability of small-size, reasonably accurate on-device models whose outputs can be effectively differentiated for samples that require remote inference. Despite the performance gains, HI requires on-device inference for all samples, which adds a fixed overhead to its latency and energy consumption. Therefore, we design a hybrid system, Early Exit with HI (EE-HI), and demonstrate that compared to HI, EE-HI reduces the latency by up to 59.7% and lowers the device's energy consumption by up to 60.4%.

==> S1.Intro_bkp12012025.tex <==
\section{Introduction}\label{sec:intro}
%Importance of on-device inference
%On-device ML inference holds great promise for real-time decision-making, enabling applications like image recognition, natural language processing, and predictive analytics to be run directly on the device. 
Deep Learning (DL) inference on data generated by \textit{end devices} such as IoT sensors, smartphones, and drones enables significant improvements in operational efficiency and functionality across various sectors, including industrial automation, smart cities, remote healthcare, smart agriculture, and other sectors. Performing DL inference locally on the device has the added advantage of increased energy efficiency \cite{banbury2021micronets}, responsiveness, and privacy and holds great promise for real-time decision-making. Thus, significant efforts have been directed towards designing and developing compact DL models specifically tailored for deployment on end devices \cite{deng2020model,chen2020deep,sanchez2020tinyml}.
%There is a significant research thrust in building tinyML models to enable complex tasks such as image classification for medical diagnosis, natural language processing for chatbots, and predictive analytics for fraud detection. 
This resulted in a plethora of DL models, such as MobileNet \cite{sandler2018mobilenetv2}, EfficientNet \cite{tan2019efficientnet}, and Gemma 2B large language model \cite{gemmateam2024}, which can be embedded on moderately powerful smartphones. Additionally, tinyML models like ResNet-8 \cite{banbury2021mlperf} have been designed for extremely resource-limited micro-controller units (MCUs). 


\begin{figure} [ht!] 
    \begin{center}
  \includegraphics[width=8.5cm]{figures/PC_MCUs.pdf}
    \end{center}
    \caption{Measured inference accuracy and latency per inference for various models on different MCUs: Arduino Nano, ESP-32, and Coral Micro, for the MNIST, CIFAR-10, and ImageNet-1K datasets. As the inference complexity increases from MNIST to ImageNet-1K, even resorting to larger DL models and powerful MCU Coral Micro (with TPU) may be insufficient to satisfy QoS requirements; for example $90$\% accuracy (green line) and $250$ ms response time (red line).} \label{fig:PC_MCUs}
\end{figure}


Especially when considering DL inference on MCUs, despite the advances in models' optimizations and improvements, the end-product use cases of on-device inference are limited to applications involving simple inference tasks -- visual keyword spotting on smartphones, gesture recognition on smart cameras, and predictive analytics for industrial machines on sensors \cite{imagimob}. 
%Given this, achieving an advantageous trade-off between accurate inference predictions and inference speed often necessitates more complex models, which are challenging to deploy on resource-limited devices. 
We indeed argue that on-device inference becomes inadequate as the complexity of the inference tasks increases. For this purpose, consider an image classification application\footnote{We focus on image classification datasets and models as they span a broad range of complexity and are widely used benchmarks for evaluating the performance of DL systems \cite{reddi2020mlperf}.} with a QoS requirement of at least $90$\% accuracy and maximum $250$ ms latency\footnote{This value is motivated by the latency requirement of $100$ to $500$ ms in real-time computer vision applications such as scene text detection \cite{zhou2017east}, and image captioning \cite{zhou2021semi}.}.
%-- where QoS entails the entire duration required for an inference task to be executed by an end device while ensuring an average accuracy above a certain threshold and within a time limit. 
In Fig. \ref{fig:PC_MCUs}, we present the accuracy and latency for different ML models on three MCUs: Arduino Nano, ESP-32, and Coral Micro (cf. Table \ref{tab:mcus}). Of the MCUs, Coral Micro is the most powerful, featuring a Tensor Processing Unit (TPU). For the inference tasks, we categorize MNIST image classification as a simple task, CIFAR-10 as a moderately complex task, and ImageNet-1K as a complex task. Observe that Arduino Nano and ESP-32 satisfy the QoS requirement for the MNIST dataset using Logistic Regression (LR). But both devices fall short of latency and accuracy requirements for CIFAR-10 dataset because running the state-of-the-art tinyML model ResNet-8, which has $87$\% accuracy, takes at least $600$ ms. Coral Micro can meet the QoS requirements for CIFAR-10, using a bigger DL model ResNet-56, but it cannot do so for ImageNet-1K. 

\begin{comment}
Arduino Nano and ESP-32 have latency within $1$ ms for running Logistic Regression (LR), which has $92.5$\% accuracy to classify an MNIST image. However, both devices have inference times greater than $600$ ms for running ResNet-8, which has $87$\%  to classify a CIFAR-10 image. Thus, these devices cannot satisfy the QoS requirements for CIFAR-10 image classification. 

One may consider the more powerful Coral Micro for classifying CIFAR-10 images. It takes $1.5$ ms to run ResNet-8, but will not meet the accuracy requirement. However, using a bigger model ResNet-56, Coral Micro meets the QoS requirements. Considering ImageNet-1K dataset, Coral Micro cannot satisfy the accuracy requirement as there are no state-of-the-art DL models that achieve higher than $90$\% accuracy for this dataset.  in the case of using ResNet-18 and both accuracy and the deadline constraint in the case of using ResNet-50. 
\end{comment}

%All three devices are inadequate for satisfying QoS requirements for ImageNet-1K. 
%Large-scale adoption of on-device inference faces serious challenges as smaller-size DL models have lower accuracy and lack generalization capability and robustness to noise. One may have to resort to large-size DL models to achieve a desirable inference accuracy, but the resource-constrained devices may be unable to load such models. Even if one chooses a moderately powerful device that can host large-size models, the computation time per inference can still be prohibitive for real-time decision-making. These issues become even more critical in the case of battery-powered devices as the energy consumed per inference increases with model size.  
%Though there are state-of-the-art compressed and optimized models designed for on-device inference, we argue that these are severely limited because of the computing and memory constraints on devices.

%Shortcomings of on-device inference


%Devices are well connected to networks
% The first sentence below sounds a bit strange, "to address the shortcomings of on-device inference, we observe..? I think this needs to be rephrased. Maybe we don't even need the first sentence because, in essence, it doesn't add much? We could instead say: "Edge devices are being increasingly exposed to good quality networks. For network-enabled devices, a simple ... I added this below to show a complete examples

%Thus, on-device inference is inadequate for several applications due to the lower accuracy of the small-size DL models or high latency if relatively larger-size models are used. Also, small-size DL models lack robustness to noisy data and generalization capability \cite{bubeck2023universal}. Furthermore, when considering battery-powered devices, typical of many IoT settings, recursively running inference tasks may impact battery life, especially when relying on more complex models. All these factors hinder the large-scale adoption of on-device inference. 

%Though the devices are becoming powerful with improved hardware, the DL inference tasks are increasingly becoming complex to be supported by the devices in a stand-alone mode. 
\jpcol{Although devices are becoming more computationally powerful due to advanced hardware, the ever increasing complexity of DL inference tasks poses significant challenges for these devices to handle them in a stand-alone mode, hindering the large-scale adoption of on-device inference.}
%The issues discussed above hinder the large-scale adoption of on-device inference. 
An alternate solution for devices connected to a network is to use an edge server/cloud that uses a state-of-the-art large-size DL model.
%Today, over $15$ billion devices are connected to the network, which is predicted to increase significantly in 6G networks. 
%end devices are being increasingly exposed to good-quality networks. 
By offloading all the samples for \textit{remote inference} on the large-size DL model, a device can achieve higher accuracy rather than inferring locally. However, fully offloading DL inference execution risks not leveraging on-device capabilities, incurs additional network latency and connectivity dependency, and forgoes the benefits of increased energy efficiency and responsiveness of on-device inference.



\begin{comment}
\begin{figure} [t!] 
    \begin{center}
  \includegraphics[width=9cm]{figures/HI_System.pdf}
    \end{center}
    \caption{Schematic of the Hierarchical Inference system.} \label{fig:HI-system}
\end{figure}
\end{comment}

%A data sample is offloaded for remote DL inference on an edge/cloud server only if the local inference is likely incorrect.  
%Such a strategy capitalizes on differentiating data samples, enabling a selective offloading approach. By differentiating early in the inference pipeline, the system dynamically decides which samples require the capabilities of the remote DL model on the edge server, optimizing resource utilization and inference accuracy on the edge device. 
%This approach aligns with the broader goal of maximizing the efficiency of ML deployments on edge devices, particularly when faced with computational constraints, and emphasizes the importance of judiciously offloading only those samples that demand the additional capabilities of the larger DL model on an edge/cloud server. 
%HI reaps the benefits of performing inference on EDs without compromising on the accuracy achieved at ESs. To see this, note that HI offloads only complex data samples that need further inference assistance and will (most likely) receive correct inference from remote ML on the edge server/cloud, while simple data samples that are either redundant or receive correct inference from local ML are not offloaded, thus saving bandwidth and reducing latency and energy for transmission and computation on L-ML.
 %It involves leveraging the differences in model sizes between the edge device and the edge server (ES) to enhance the efficiency of the inference process. The edge device hosts a relatively compact ML model termed S-ML, while the ES boasts a more substantial and advanced model known as L-ML. The key proposition is to identify complex samples early in the on-device inference using the smaller local MLmodel. If it is determined that the local MLinference is insufficient for accurate predictions on a particular sample, the system can promptly offload that sample to the ES for processing with the more sophisticated remote MLmodel.

%HI systems has received considerable attention in the recent past~\cite{Nikoloska2021,Ghina2023,behera2023,Moothedath2024,Beytur2024}. These works used soft-max values output by the local DL model to differentiate the simple and complex samples and demonstrated a significant increase in the accuracy achieved by HI compared to on-device inference. 

In this context, Hierarchical Inference (HI) \cite{Moothedath2024} has recently emerged as a novel distributed ML inference technique that mitigates the limitations of on-device inference by using remote inference when necessary. Under a HI system, inference is performed first on the local DL model for each data sample. A data sample for which the local inference is likely correct is a \textit{simple data sample}, and its inference is accepted, while a data sample for which the local inference is likely incorrect is a \textit{complex data sample}, which is offloaded. 
By only offloading the complex samples, HI reaps the benefits of performing inference on end devices without compromising on accuracy, and thus, it received considerable attention in the recent past~\cite{Nikoloska2021,Ghina2023,behera2023,Moothedath2024,Beytur2024}.

HI operates through a decision algorithm that acts on the on-device (local ML) model output for each input sample and decides whether to accept the local inference or offload the sample. Consequently, HI requires on-device inference for every sample, introducing a fixed overhead to latency and energy consumption per inference. However, all the existing work on HI only studied the accuracy improvement over the on-device inference without accounting for its latency and on-device energy consumption overheads. Further, their conclusions were based only on simulations using abstract costs for offloading and misclassification errors. Additionally, they ignore the diversity and heterogeneity of edge ML systems, including varying hardware, network connectivity, and models. 

In this paper, we address the above shortcomings and make multiple contributions. We perform accuracy, latency, and energy measurements for running embedded DL models on five devices with different capabilities and three image classification datasets (please refer to Section \ref{sec:system} for additional details about the devices and models used). These measurements will be of independent interest to the embedded ML community. Using the measurements, we empirically evaluate the performance of HI and on-device inference and demonstrate that HI improves accuracy but has higher latency and energy consumption. This raises the question of the true benefits of using HI. We answer this question in light of QoS requirements. 
We demonstrate that a HI system achieves a given accuracy requirement using a small on-device model, even if this model's accuracy is below the specified requirement. Consequently, the HI system using the small model achieves lower latency and energy consumption than a larger on-device model that meets the initial accuracy requirement. This establishes the benefit of using HI over on-device inference.
%Given an accuracy requirement, we demonstrate that HI achieves t using a smaller on-device model (even if its accuracy is below the specified requirement) results in a lower latency and energy consumption than a larger on-device model that meets the initial accuracy requirement.
%a key insight we provide is that, given an accuracy requirement, the latency and energy overheads of a HI system can be reduced by using a smaller on-device model (whose accuracy can be lower than the accuracy requirement). 
For instance, on the Raspberry Pi, with an accuracy requirement of $90$\% for CIFAR-10 image classification, we demonstrate that using a smaller model, ResNet-8, with HI achieves $95.9$\% accuracy and has $73$\% lower latency and $77$\% lower energy consumption than the on-device larger model, ResNet-56, with $93.7$\% accuracy. Additionally, HI achieves up to $11$\% (absolute difference) higher accuracy for a given latency and energy requirement for the systems we studied.
%Similarly, on Coral Micro, for an accuracy requirement of $81$\% for ImageNet-1K, ResNet-18 with HI achieves $85.2$\% accuracy and has $70.5$\% lower latency and $69.25$\% lower energy consumption than the on-device inference using ResNet-50. 

%This raises the question: \textit{given an on-device inference system that achieves an accuracy QoS requirement, can we design an HI system that achieves the accuracy QoS requirement but has faster responsiveness and lower on-device energy consumption?} 
%To answer this question, we performed accuracy, latency, and energy measurements for running embedded DL models on five devices with different capabilities and three image classification datasets (please refer to Section \ref{sec:system} for additional details about the devices and models used).
%various devices for multiple datasets MNIST, CIFAR-10, and . 
%Specifically, the measurements are performed on two types of devices: 1) MCUs (Arduino Nano BLE sense, ESP-32, and Coral Micro) and 2) single-board computers (Raspberry Pi and Jetson Orin). These devices cover different processing units: CPU, GPU, and TPU, thus providing heterogeneity in the measurements. 
%For the application, we study image classification, where the complexity of the task is categorized based on the dataset we choose. 
%We choose MNIST as the simple task, CIFAR-10 as a moderately complex task, and ImageNet-1K as the complex task. 
%The ML models we use are the well-established models: Logistic Regression (LR), ResNet-8, ResNet-18, ResNet-50, ResNet-56, and AlexNet. 
%The performance measures we use to compare different methods are accuracy, the latency per inference, and energy per inference.

%In the empirical evaluation, we compared the performance of HI with on-device inference. For a given accuracy requirement, efficient HI systems can be designed to achieve lower latency, up to $73$\% reduction, and lower device energy consumption, up to $77$\% reduction, compared to an on-device inference system in a wide range of scenarios. 
However, for ImageNet-1K image classification, offloading for remote inference remains the only viable solution on Coral Micro and Raspberry Pi due to the lack of on-device models that can provide the necessary lower latency and energy consumption. 
%An important observation we make is that, in contrast to on-device inference, HI does not require large-size on-device models to meet high accuracy QoS requirements; rather, the model should be small in size, and its output can be effectively used to differentiate between simple and complex samples. This calls for the design of small-size, reasonably accurate embedded ML models whose outputs are better calibrated for differentiating between simple and complex samples.
%Thus, the key to building an efficient HI system is the availability of a smaller-size local ML with reasonable accuracy. 
%This calls for the design of embedded ML models that do not need to compete with state-of-the-art large-size DL models in terms of accuracy but are more efficient regarding their accuracy-to-size ratio. 
To alleviate this issue, we resort to the early exit technique \cite{teerapittayanon2016branchynet}, which improves HI by reducing the latency of the on-device inference. Using this technique, we design a hybrid system, Early Exit with HI (EE-HI), and demonstrate that compared to HI, EE-HI reduces the latency up to $59.7$\% and the device's energy consumption up to $60.4$\%.
%on Jetson Orin for CIFAR-10 image classification.

The rest of the paper is organized as follows. In Section \ref{sec:related}, we discuss the related works and the existing edge ML inference strategies.
In Section \ref{sec:system}, we describe the system methodology used for measurements. 
%In Section \ref{sec:measuremet_results} we discuss the details of the measurement setup on different devices. 
We present the measurement results in Section \ref{sec:measuremet_results}, and compare the performance of HI, on-device, and remote inference in Section \ref{sec:comparison}. We present the design and the results of EE-HI in Section \ref{sec:EEHI} and conclude in Section \ref{sec:conclusion}. 

\begin{comment}
Our main contributions are summarized below:
\begin{itemize}
    \item We present energy, latency, and accuracy measurement for ML inference on five devices, ranging from a highly resource-constrained MCU to a moderately powerful device with GPU, encompassing the heterogeneous processing units: CPU, GPU, and TPU.
    \item Using the measurements, we demonstrate that using HI with the state-of-the-art local ML increases accuracy, but it also results in an increase of energy per inference and latency per inference, and thus, it may violate the QoS constraints. Interestingly, using HI with a smaller-size local ML instead of the state-of-the-art local ML achieves the required accuracy requirement while reducing the energy and latency compared to the standalone state-of-the-art local ML in many scenarios. 
    
    Thus, HI favors relatively smaller-size local ML models, calling for the design of on-device ML models that do not need to compete with the remote ML models in terms of accuracy but rather provide reasonable accuracy while being small-size.
    
    \item We also design and train compact DL models with early-exit technique and demonstrate that this further enhances the improvements achieved by HI.
\end{itemize}
\end{comment}

% TODO: outline the structure of the paper.

%According to the IoT device categorization is done by IETF RFC 772
%https://www.ietf.org/archive/id/draft-bormann-lwig-7228bis-08.html#name-classes-of-constrained-devi

%Arduino Nano 33 BLE sense
%64 MHz Arm® Cortex®-M4F (with FPU)
%1 MB Flash + 256 KB RAM

%ESP32 
%240 MHz Xtensa® 32-bit LX6 microprocessor
%8 MB Flash + 520 KB RAM



==> S4.Measurements_bkp30062024.tex <==
\section{Measurements: Server and Wireless Communication Times}
We have considered a pre-trained ViT-H/14 \cite{dosovitskiyimage}, which we fine-tuned up to $98.77\%$ accuracy, as our remote model for CIFAR-10. Similarly, for ImageNet-1K, we have considered a ConvNeXT \cite{liu2022convnet} with $86.58\%$ accuracy. We tested our remote models using two distinct servers with different GPUs: NVIDIA Tesla T4 and NVIDIA A100. For the former, we measured an averaged time per inference of 19.18ms for CIFAR-10 and 12.01ms for ImageNet-1k. For the latter, the measured times were: 4.29ms for CIFAR-10 and 4.41ms for ImageNet-1k. These numbers were obtained using half precision (FP16), a format that uses 16 bits to represent floating-point numbers. Both GPUs have specialized hardware for FP16 arithmetic, which increased performance with negligible accuracy loss. During integration in the final system, we recorded an average time for completion of an inference request of 6.95 ms for CIFAR-10 and 5.08 ms for Imagenet-1k. The reason for this is that ConvNeXT uses the same input as the edge models. Therefore, when the image is received by the server, we can immediately perform preprocessing, which took an average of 0.7 ms on the GPU. However, preparing data for ViT-H/14 is more involved as it entails the transposition of the input buffer to NCHW format and upscaling to the appropriate dimensions before we can proceed with preprocessing. The additional operations are accountable for the uneven increase in the total execution time compared to ConvNeXT.

Considering that both devices are equipped with NVIDIA hardware, TensorRT was deemed the optimal choice for conducting inference testing. Nonetheless, the size of ViT-H/14 exceeds the 2 GB restriction in the protobuf serialized message size, rendering it impossible to parse the model into the framework. Instead, the ONNX Runtime was utilized with the CUDA execution provider, given that TensorRT execution provider naturally fails in this framework for the same reason. However, the ConvNeXT model did not have this issue and the inference was executed using TensorRT execution provider within ONNX Runtime.


\subsection{Wireless communication timings:}

\subsubsection{Communication protocol comparison:}
Given the availability of both BLE and Wi-fi for most of the tested devices, the question of which one should be used arises. To address it, an experiment is performed on a Raspberry pi where both latency and energy are measured for the transmission of a CIFAR-10 image.

As expected, the power demands for BLE are smaller. From 2.23 W to 2.71W measured for Wi-fi. However, when the latency factor is considered to compute the energy consumption per transmitted image, results differ. On the one hand, on average, transmitting an image to the server and receiving two bytes back consumes 7.39 mJ in the case of Wi-fi. On the other, the same process for BLE consumes 395 mJ. 

Given the significant differences in terms of both latency and energy, we opt for a Wi-fi implementation where possible.

\subsubsection{Implementation:}
In order to assess the expenses associated with the offloading process, we have quantified the duration required to transmit an image over Wi-Fi and getting a response back. The edge device, operating as a client, transmits a request to the server that is actively monitoring communications. 

In order to establish Wi-Fi connectivity, the client connects to a hotspot that access the local network where the server is operating. The experiment was designed to transmit an image as a raw byte array via TCP and receive a number representing the anticipated class by performing inference on the server using the incoming array. The duration between the initiation of the offload process and the reception of the response is repeatedly assessed to eliminate the significant fluctuations commonly observed in WiFi communications.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Latency and energy required to offload an image to the server and wait until the prediction from the larger model is received}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll|l|l|ll|}
\cline{3-6}
                                                         &                  & \multirow{2}{*}{\textbf{Coral}} & \multirow{2}{*}{\textbf{RPi}} & \multicolumn{2}{l|}{\textbf{Jetson Orin}}      \\ \cline{5-6} 
                                                         &                  &                                 &                                     & \multicolumn{1}{l|}{\textbf{LP}} & \textbf{HP} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{CIFAR-10}}} & \textbf{Latency (ms)} & 10.37                           & 9.68                                & \multicolumn{1}{l|}{8.34}        & 8.20        \\ \cline{2-6} 
\multicolumn{1}{|l|}{}                                   & \textbf{Energy (mJ)}  & 14.61                           & 27.67                               & \multicolumn{1}{l|}{50.48}        & 55.91        \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{ImageNet}}} & \textbf{Latency (ms)} & 84.41                           & 28.74                               & \multicolumn{1}{l|}{16.42}       & 16.45       \\ \cline{2-6} 
\multicolumn{1}{|l|}{}                                   & \textbf{Energy (mJ)}  & 145.13                          & 112.01                              & \multicolumn{1}{l|}{111.57}        & 124.93        \\ \hline
\end{tabular}
}

\label{off_table}
\end{table}


In Table \ref{off_table}, one can see the time and energy costs per offloaded image. This measurement includes sending the image to the remote server and waiting for the output of the remote model to be received on the device.

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{comment}
\begin{table}[H]
\caption{\JP{Add these values in text?} Average execution time in milliseconds for the models in the server for different hardware. Both use FP16 precission.}
\label{tab:latency-server}
\centering
%\resizebox{\columnwidth}{!}{%


\begin{tabular}{c|c|c|}
\cline{2-3}
                                          & \textbf{T4} & \textbf{A100} \\ \hline
\multicolumn{1}{|c|}{\textbf{CIFAR-10}}   & 19.1758     & 4.2908        \\ \hline
\multicolumn{1}{|c|}{\textbf{ImageNet1k}} & 12.0990     & 4.4127        \\ \hline
\end{tabular}%
%}
\end{table}
\end{comment}

%Avg inference time (T4 onnxruntime): 17.599645137786865 ms  19.17585015296936 ms
%Avg inference time (A100 onnxruntime): 4.320067310333251 ms

\section{Measurements on Devices}
%\JP{Please mention key challenges faced in obtaining the measurements. There can be an overview of the challenges at the start of the section and also specific challenges faced in each subsection corresponding to each device.}

The measurement code infrastructure for each of the selected devices had distinct implementations due to varying device characteristics and supported underlying technology stacks. All devices used models that have undergone compression using \texttt{INT8} quantization. These models are used due to minimal accuracy loss, improved performance, energy consumption and memory footprint. In this section, we elaborate on the implementation intrinsics for each device and the obtained measurements.




\subsection{Arduino Nano 33 BLE Sense}\label{sec:nano33}

Arduino Nano is the least powerful device tested which leads to slower on-device computation. Furthermore, contrary to all other devices, it does not support Wi-fi communication. For this reason, in case of offload, the images are transmitted to the edge server via Bluetooth Low Energy (BLE). 

On-device inference is performed using the TensorFlow Lite Micro framework, which requires loading the model as a binary file. For the decision module, the two highest per class confidence values are retrieved and multiplied by the appropriate weights to obtain the output of logistic regression. All the implementation code is written in C.

Regarding the communication aspect, Arduino provides its own BLE library \footnote{https://www.arduino.cc/reference/en/libraries/arduinoble/}, which can be used to implement both a peripheral and a central device. For this application, it was only used to build the peripheral side on the edge device. For the central role, a multi-platform library called \texttt{SimpleBLE}\footnote{https://github.com/OpenBluetoothToolbox/SimpleBLE} was used, although some other options are available depending on the specifics of the device. Since both devices allow it, the 5.0 version of the BLE protocol was used. Several modifications can be applied to the protocol which affect both the throughput and the power consumption of the application such us: connection interval, PHY, maximum transmission unit and operation type. An important requirement of this application is the absence of lost packets during transmission, as the edge server model needs the whole image to perform inference. Ensuring this compromises the throughput of the application by limiting the operation types used or requiring the addition of delays. 

Table \ref{mcus_c10} presents the accuracy and time per inference for CIFAR-10. Device refers to on-device only while system refers to an HI implementation. Offload integrates communication time and server inferene time. It can be observed that for both devices, performing inference locally is outside the QoS in terms of accuracy and, especially, in terms of latency. These results support the argument made in the introduction against on-device inference on MCUs (without hardware accelerators) for complex tasks. 





\begin{comment}
Wireless communication timing disclaimer:
Work in progress. For now, between 150 and 200 ms. per sample. This time includes the addition of delays after each characteristic is written on the peripheral side. Without those, the image is not received entirely on the central device. This results considers the default 1M PHY. If both devices support Bluetooth 5.0 (or later versions), a faster 2M PHY could be accessed depending on the frameworks and libraries being used.


\subsubsection{Mnist}

Here, the model deployed is a simple logistic regression with softmax activation. The accuracy of the quantized model deployed on the device is 91.37\%  and the average inference latency is 0.87 ms.



\subsubsection{CIFAR-10}
\end{comment}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht]
\caption{ResNet-8 on CIFAR-10 results for Arduino Nano and ESP-32. }
\begin{tabular}{ll|ll|}
\cline{3-4}
                                                         &                       & \multicolumn{1}{l|}{\textbf{Arduino}} & \textbf{ESP-32} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Accuracy}}} & \textbf{Device}       & \multicolumn{2}{l|}{87.07}                              \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                   & \textbf{System (off)} & \multicolumn{2}{l|}{95.75 (21.57)}                      \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Latency (ms)}}}      & \textbf{Device}       & \multicolumn{1}{l|}{1230.48}          & 602.52          \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                   & \textbf{Offload} & \multicolumn{1}{l|}{190.35}                 &       10.10          \\ \hline
\end{tabular}
\label{mcus_c10}
\end{table}


\begin{comment}
    \begin{table}[h]
\centering
\begin{tabular}{l|l|}
\cline{2-2}
       & \textbf{Time ($ms$)}    \\ \hline
%\multicolumn{1}{|l|}{LR}       & 0.055 \\ \hline
\multicolumn{1}{|l|}{TinyML}   & 1230.477 \\ \hline
\multicolumn{1}{|l|}{Complete} & 1231.380 \\ \hline
\end{tabular}
\caption{Time measurements without communication for Resnet8 on Arduino device }
\end{table}
\end{comment}




  










\subsection{ESP32}

% The XTensa microprocessor incorporates a set of Single Instruction, Multiple Data (SIMD) instructions that can enhance the performance of machine learning workloads.  An example is the vectorized fused multiply and add on 8 bit data, which includes loading the preceding data and ensuring alignment. This is especially advantageous for quantized convolutions and fully connected layers and may be a major contributor to the substantial enhancement in performance observed in quantized models. Even if a high level API is being used and the compiler misses the SIMD optimizations, it will still mean a greater proportion of the network fits into the cache lines. This, in turn, will reduce cache misses, which are costlier than arithmetic operations.

In order to exploit all the functionality and performance available on the ESP32-DevKitC V4, Espressif IoT Development Framework (ESP-IDF) has been used. For on-device inference, the same rationale exposed in \ref{sec:nano33} applies to this case.

For wireless communications via WiFi, the ESP32 requires specific setup to get as close to the theoretical maximum throughput as possible. Some settings were taken from the \texttt{iperf} example application, such as TCP buffer sizes, lwIP task and mailbox sizes, lwIP IRAM optimization, lwIP TCP/IP task priority and Wi-Fi buffer configuration. Refer to the Github repository \footnote{https://github.com/JoseGaDel/DIME.git} for a more detailed explanation of this configuration.

% Depending on how congested the channels are, average transfer times may vary between \textbf{2.8} and \textbf{3.4} milliseconds.


\begin{comment}
    

Three measurements have been taken reading from hardware counters to achieve high precision with low overhead. One for inference, of the tinyML model, another for LR and one including the whole process. The results from averaging over 1000 CIFAR-10 images are:


\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc}
\hline
\multicolumn{1}{|c|}{\textbf{Good predictions}} & \multicolumn{1}{c|}{\textbf{Bad predictions}}        & \multicolumn{1}{c|}{\textbf{Precision ($\%$)}}          \\ \hline
\multicolumn{1}{|c|}{970}                       & \multicolumn{1}{c|}{30}                              & \multicolumn{1}{c|}{97.0}                               \\ \hline
\multicolumn{1}{l}{}                            & \multicolumn{1}{l}{}                                 & \multicolumn{1}{l}{}                                    \\ \hline
\multicolumn{1}{|c|}{\textbf{Num. Offloads}}    & \multicolumn{1}{c|}{\textbf{Correct LR predictions}} & \multicolumn{1}{c|}{\textbf{Precision without offload}} \\ \hline
\multicolumn{1}{|c|}{233}                       & \multicolumn{1}{c|}{90}                              & \multicolumn{1}{c|}{88.0}                               \\ \hline
\end{tabular}%
}
\caption{Precision of running inference on the ESP32 for 1000 images.}
\label{tab:esp32infer}
\end{table}



\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccl}
\hline
\multicolumn{1}{|c|}{\textbf{Avg inference time (s)}} & \multicolumn{1}{c|}{\textbf{Avg LR time (s)}}  & \multicolumn{1}{c|}{\textbf{Avg total time (s)}} \\ \hline
\multicolumn{1}{|c|}{0.602724746}                     & \multicolumn{1}{c|}{6.9575e-05}                & \multicolumn{1}{c|}{0.603142045}                 \\ \hline
\multicolumn{1}{l}{}                                  & \multicolumn{1}{l}{}                           &                                                  \\ \cline{1-2}
\multicolumn{1}{|c|}{\textbf{Fraction infer time}}    & \multicolumn{1}{c|}{\textbf{Fraction LR time}} &                                                  \\ \cline{1-2}
\multicolumn{1}{|c|}{$99.930 \%$}                     & \multicolumn{1}{c|}{$0.011 \%$}                &                                                  \\ \cline{1-2}
\end{tabular}%
}
\caption{Average latency for performing inference over 1000 images fro the CIFAR-10 dataset. The last two values show which fraction of the total execution time each stage represents.}
\label{tab:esp32infertime-cifar}
\end{table}

\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccl}
\hline
\multicolumn{1}{|c|}{\textbf{Avg inference time (s)}} & \multicolumn{1}{c|}{\textbf{Avg LR time (s)}}  & \multicolumn{1}{c|}{\textbf{Avg total time (s)}} \\ \hline
\multicolumn{1}{|c|}{0.0005901036}                     & \multicolumn{1}{c|}{2.41728e-05}                & \multicolumn{1}{c|}{0.0006274392}                 \\ \hline
\multicolumn{1}{l}{}                                  & \multicolumn{1}{l}{}                           &                                                  \\ \cline{1-2}
\multicolumn{1}{|c|}{\textbf{Fraction infer time}}    & \multicolumn{1}{c|}{\textbf{Fraction LR time}} &                                                  \\ \cline{1-2}
\multicolumn{1}{|c|}{$94.049 \%$}                     & \multicolumn{1}{c|}{$3.853 \%$}                &                                                  \\ \cline{1-2}
\end{tabular}%
}
\caption{\JP{Redundant:} Average latency for performing inference over 1000 images for the MNIST dataset. The last two values show which fraction of the total execution time each stage represents.}
\label{tab:esp32infertime-mnist}
\end{table}

\end{comment}

==> S6.EEHIbkp28062024.tex <==
\section{Early Exit with HI}
%\AB{Write from QoS POV}
%As discussed before, maintaining QoS is essential in resource-constrained IoT networks, particularly those engaged in image classification tasks. 
As a case study, we consider a QoS requirement to achieve $90\%$ of the accuracy of the remote ML model while balancing latency and energy efficiency. Although local ML models like ResNet-8 for the CIFAR-10 dataset and ResNet-18 for the ImageNet-1K dataset achieve reasonably high accuracy with lower latency and energy per inference, they fail to meet this accuracy requirement through on-device inference alone. 
HI helps to increase the accuracy but adds additional latency and energy consumption due to extra inferences. 

%Additionally, a high number of false negatives, where simple samples are unnecessarily offloaded to the server for further inference, increases the number of redundant inferences which requires higher latency and energy requirements. 

Keeping this in mind, we propose a novel strategy incorporating Early Exit with HI (EE-HI) that presents a promising approach to optimize the performance of image classification tasks in IoT environments, particularly leveraging datasets like CIFAR-10 where simple samples outnumber complex ones. These simple samples usually do not require going through all the layers of the local DL model to obtain accurate inference results. EE-HI integrates early exit branches in the intermediate layers of the DL model, allowing the local ML model to make confident predictions for simple samples without processing all the layers. This early identification and acceptance of simple samples significantly reduce latency and energy consumption per inference, which is crucial for real-time applications.

EE-HI effectively prioritizes computational resources by implementing early exit points, ensuring that local devices focus on complex data samples that genuinely require further analysis. This optimization enhances the efficiency of HI system by reducing the overall latency and energy consumption. For samples that require further validation or analysis after the initial on-device inference, EE-HI employs a decision module, such as a predefined confidence threshold or a pre-trained logistic regression, to determine whether offloading to a more powerful server is necessary, as shown in Figure \ref{fig:EEHI_EA}\JP{Explain more}. This approach not only meets the stringent QoS requirements demanded by IoT networks but also ensures efficient resource utilization and improved overall system performance in dynamic and resource-constrained environments.




\begin{comment}
Keeping this in mind, we propose a novel strategy incorporating early exit with HI (EEHI), where simple samples can be identified and exited early in the network while doing on device inference. Usually, in datasets like CIFAR-10, the number of simple samples is much higher in comparison to the number of complex samples. These simple samples usually do not require to go through the entire DL model in order to get an inference. Many of these simple samples can be identified early by incorporating an exit branch mid way through the DL model, where if a confident prediction can be made, we accept the inference as a correct inference and do not let it run on the entire DL model. This in turns reduces latency and energy requirement per inference. However, if a confident prediction can not be made, the data sample is allowed to run its course through on device inference and after the final layer (or final exit) we assess the prediction to see whether it needs further help from the remote server or not through our predefined LR model as the decision module. So, in short we incorporate early exit into HI strategy to identify and accept simple samples early and through early exit and offload complex samples after the on device inference for further help.

\begin{figure} [ht!] 
    \begin{center}
  \includegraphics[width=8.5cm]{figures/Early_Acceptance.png}
    \end{center}
    \caption{Early Exit with HI in modified ResNet-8} \label{fig:EEHI_EA}
\end{figure}

\end{comment}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{ Results for the EE-HI system with optimal threshold
subject to a QoS requirement on accuracy of at least
90\% of the SOTA. Last two columns represent the measurements for HI implmentations for the sake of comparison.} 
\tiny
\begin{tabular}{lll|l|l|l|l|l|l|}
\cline{4-9}
                                                          &                                                       &             & \textbf{Threshold ($\theta^{*}$)}                 & \textbf{Acc}           & \textbf{TPI} & \textbf{EPI} 

                                                           & \textbf{TPI(HI)} & \textbf{EPI(HI)} 
                                                          \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Resnet-8}}}  & \multicolumn{2}{l|}{\textbf{Raspi}}                                 & \multirow{3}{*}{0.64}      & \multirow{3}{*}{89.01} & 2.70         & 9.00      &3.82  &12.55   \\ \cline{2-3} \cline{6-9} 
\multicolumn{1}{|l|}{}                                    & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Jetson}}} & \textbf{LP} &                            &                        & 1.38         & 8.54     &2.04  &12.57         \\ \cline{3-3} \cline{6-9} 
\multicolumn{1}{|l|}{}                                    & \multicolumn{1}{l|}{}                                 & \textbf{HP} &                            &                        & 1.28         & 8.98    &1.87  &13.05     \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{ResNet-56}}} & \multicolumn{2}{l|}{\textbf{Raspi}}                                 & \multirow{3}{*}{0.77, 
 0.81} & \multirow{3}{*}{88.91} & 5.56         & 20.85  &15.21  &58.10      \\ \cline{2-3} \cline{6-9} 
\multicolumn{1}{|l|}{}                                    & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Jetson}}} & \textbf{LP} &                            &                        & 0.76         & 4.96     &1.67  &10.95    \\ \cline{3-3} \cline{6-9} 
\multicolumn{1}{|l|}{}                                    & \multicolumn{1}{l|}{}                                 & \textbf{HP} &                            &                        & 0.62         & 4.67       &1.24  &9.63  \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{AlexNet}}}   & \multicolumn{2}{l|}{\textbf{Raspi}}                                 & \multirow{3}{*}{0.70}      & \multirow{3}{*}{88.95} & 5.25         & 18.13      &7.81  &28.22  \\ \cline{2-3} \cline{6-9} 
\multicolumn{1}{|l|}{}                                    & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Jetson}}} & \textbf{LP} &                            &                        & 2.44         & 15.51      &3.27  &21.59  \\ \cline{3-3} \cline{6-9} 
\multicolumn{1}{|l|}{}                                    & \multicolumn{1}{l|}{}                                 & \textbf{HP} &                            &                        & 2.27         & 16.26     &2.90  &21.53   \\ \hline
\end{tabular}
\label{EEHI}
\label{tab: EE_thresholds}
\end{table}

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]
    {Inaki/EEresnet8.png}
    \caption{Comparison of different approaches with Resnet8 as base model for Raspberry}
    \label{fig:EEHI_Res8}
\end{figure}
\end{comment}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]
    {Inaki/EEalexnet.png}
    \caption{ Comparison of different approaches with
AlexNet as base model for Raspberry. A QoS of at least 90\% of the accuracy of the SOTA model is required.}
    
    \label{fig:EEHI_Alex}
\end{figure}

\begin{comment}
    

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]
    {Inaki/EEresnet56.png}
    \caption{ Comparison of different approaches with
ResNet56 as base model for Raspberry. A QoS of at least 90\% of the accuracy of the SOTA model is required. The blue and orange dots are obtained fixing $\theta_{1} = 0.77$ an varying $\theta_{2}$  \textcolor{red}{Check next figure. Is it a good idea to plot some combinations which do not contain the optimal for the QoS to show the huge variability when two thresholds need to be chosen?}}
    
    \label{fig:EEHI_Res562}
\end{figure}
\end{comment}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]
    {Inaki/EEresnet562.png}
    \caption{ Comparison of different approaches with
ResNet56 as base model for Raspberry. A QoS of at least 90\% of the accuracy of the SOTA model is required. The dark blue and orange dots are obtained fixing $\theta_{1} = 0.77$ an varying $\theta_{2}$. The lighter colors are obtained fixing $\theta_{1} = 0.95$ and varying $\theta_{2}$, to show the flexibility of the model with multiple branches}
    
    \label{fig:EEHI_Res56}
\end{figure}


In Table \ref{EEHI}, we demonstrate the effectiveness of the EE-HI strategy in meeting a QoS requirement for CIFAR-10 image classification: achieving an overall system accuracy above 90\% of the state-of-the-art remote ML model ViT-H/14 with accuracy 98.77\%, which translates to 88.9\%. The table presents the optimal threshold for the decision module to accept simple samples early for each model and the corresponding system accuracies. It can be observed that the latency and energy consumption for EE-HI in each model are lower than those of the base model with HI when using logistic regression as the decision module. \textcolor{red}{Notably, the lowest possible latency and energy consumption for this QoS requirement is achieved by ResNet-56 with EE-HI on Jetson Orin in high power mode. This performance is even better than the on-device ResNet-56 implementation for the same device and power mode, which was previously the preferred strategy for the same workloads and QoS requirements as shown in Table \ref{Req_QoS}.} 


However, HI can also have the option of choosing an optimal threshold instead of logistic regression as the decision module, which will enable it to have the flexibility of having lower latency and energy as per the QoS requirements. Figure \ref{fig:EEHI_Res8}, \ref{fig:EEHI_Alex} and \ref{fig:EEHI_Res56} shows the performance of base model with HI (both with a range of varying threshold and logistic regression as decision module) and EE-HI along with early exit for the QoS requirement discussed earlier. Although early exit on its own has much lower latency, it fails to achieve the required accuracy in both the cases. However, when EE-HI is concerned completely different trends can be observed in both the cases. In case of ResNet-8, base model with HI (optimal threshold as decision module) outperformed EE-HI, however for Alexnet, and ResNet-56, EE-HI performs much better than that of its counterpart.




It is worth mentioning that we have implemented our early exit strategy using the BranchyNet approach \cite{teerapittayanon2016branchynet}, which is the pioneer work in early exit. This approach results in improved latency and energy efficiency during on-device inference, with some reduction in the overall accuracy of the DL model. ResNet-8, being a relatively small DL model with only three residual blocks (six convolutional blocks in total), does not accommodate the addition of convolutional blocks in the early exit branch without compromising the model's primary purpose of maintaining a smaller size. This limitation leads to a reduction in overall accuracy (around 3\%). However, for larger models like ResNet-56 and AlexNet, we demonstrated that EE-HI works successfully, maintaining the benefits of early exit while preserving high accuracy.




\subsection{Limitations and future work}
Although the proposed EE-HI strategy looks promising, our implementation has certain limitations, that we would like to highlight and also discuss possible solutions to these limitations as our probable future works.

\begin{itemize}
    \item We used BranchyNet approach for early exit, which although the pioneering work in this field of study, is not the most sophisticated approach for early exit. Later approaches like self distillation \cite{zhang2021self} shows remarkable improvement in early exit implementation that not only reduces latency and energy consumption but also improve the accuracy as compared to the base model.

    \item Although EE-HI was shown to be the likely choice for bigger models, for smaller models like ResNet-8 (also known as tinyML models) early exit does not work well due their extremely small architecture (in this case only 3 residual blocks or 6 convolutional blocks) that is more beneficial to execute on-device. However, there are some recent studies \cite{ghanathe2024qute} that have been shown to be effective even for tinyML models.
    
    \item TPUs do not support customized conditional statement inside DL model architecture, hence we could not implement EE-HI for Coral Dev Micro device. 


    \item Using this current approach, we were able to train DL models for CIFAR-10 image classification without much accuracy loss. However, this approach is not suitable for bigger datasets such as ImageNet-1K as we incurred substantial accuracy loss on all the base models ResNet-18, ResNet-50, and AlexNet (5-9\%). We believe choosing  self distillation \cite{zhang2021self} as our early exit approach will solve this issue.
\end{itemize}








\begin{comment}
\begin{figure} [t!] 
    \begin{center}
  \includegraphics[width=8.5cm]{figures/Early_Rejection.png}
    \end{center}
    \caption{Early rejection with HI in modified Resnet-8} \label{fig:EEHI_ER}
\end{figure}



\subsection{Accuracy}
We implemented early offload technique on modified Resnet-8 and 







\begin{table}[ht]
\caption{Accuracy on CIFAR-10 dataset using different methods}
	\label{fig:Running time}
\tiny
\begin{tabular}{ |c||c|c|c|c|c| }
\hline
 \multicolumn{6}{|c|}{Overall System Accuracy} \\
 \hline
 
\hline
		\textbf{Methods $\rightarrow$} & 
		{\textbf{\begin{tabular}[c]{@{}c@{}}Base Model\end{tabular}}} &{\textbf{\begin{tabular}[c]{@{}c@{}}BranchyNet\end{tabular}}} & {\textbf{\begin{tabular}[c]{@{}c@{}}Base model\\ + HI\end{tabular}}} & {\textbf{\begin{tabular}[c]{@{}c@{}}Early Exit \\ + HI\end{tabular}}}
		& {\textbf{\begin{tabular}[c]{@{}c@{}}Early \\ Offload \end{tabular}}}\\   \cline{1-1}
		\textbf{Models $\downarrow$}   &   & &   &&                                                                      \\ \hline 
 
AlexNet & 74.44 & 77.20 & 90.07 & 91.2 & - \\
 \hline 

ResNet-8 & 86.81 & 85.93 & 96.57 & 98.0 & 96.67\\
\hline

ResNet-56 & 93.77 & 91.26 & 96.89 & 98.3 & - \\
\hline

 \hline
\end{tabular}
\end{table}
\end{comment}


==> To_Do.tex <==
\begin{table*}
\tiny
\caption{Tasks completed and remaining}
	\label{fig:ttc10}
\centering
\begin{tabular}{ |p{1cm}||p{1.2cm}|p{1cm}|p{1cm}|p{1cm}|p{1.2cm}|p{1.2cm}| }
\hline
 \multicolumn{7}{|c|}{CIFAR-10 Task Tracker} \\
 \hline
 
\hline
		\textbf{Tasks $\rightarrow$} & 
		{\textbf{\begin{tabular}[c]{@{}c@{}}Base Models\\Unquantized\end{tabular}}} &{\textbf{\begin{tabular}[c]{@{}c@{}}Base Models\\ Quantized\end{tabular}}} & {\textbf{\begin{tabular}[c]{@{}c@{}}Early Exit \\ + HI\end{tabular}}}
		& {\textbf{\begin{tabular}[c]{@{}c@{}}Early \\ Offload \end{tabular}}} &
        {\textbf{\begin{tabular}[c]{@{}c@{}} Time \\ Measurements \end{tabular}}} & {\textbf{\begin{tabular}[c]{@{}c@{}} Energy \\ Measurements\end{tabular}}} 
  \\   \cline{1-1}
		\textbf{Models $\downarrow$}   &   & &   &&&                                                                         \\ \hline 
 
AlexNet & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & - \\
 \hline 

ResNet-8 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark\\
\hline

ResNet-56 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & - \\
\hline

 \hline
\end{tabular}
\end{table*}


\begin{table*}
\tiny
\caption{Tasks completed and remaining}
	\label{fig:ttin}
\centering
\begin{tabular}{ |p{1cm}|p{1cm}|p{1.2cm}|p{1cm}|p{1cm}|p{1cm}|p{1.2cm}|p{1.2cm}| }
\hline
 \multicolumn{8}{|c|}{Imagenet Task Tracker} \\
 \hline
 
\hline
		\textbf{Tasks $\rightarrow$} & 
        {\textbf{\begin{tabular}[c]{@{}c@{}}Devices\end{tabular}}} &
		{\textbf{\begin{tabular}[c]{@{}c@{}}Base Models\\Unquantized\end{tabular}}} &{\textbf{\begin{tabular}[c]{@{}c@{}}Base Models\\ Quantized\end{tabular}}} & {\textbf{\begin{tabular}[c]{@{}c@{}}Early Exit \\ + HI\end{tabular}}}
		& {\textbf{\begin{tabular}[c]{@{}c@{}}Early \\ Offload \end{tabular}}} &
        {\textbf{\begin{tabular}[c]{@{}c@{}} Time \\ Measurements \end{tabular}}} & {\textbf{\begin{tabular}[c]{@{}c@{}} Energy \\ Measurements\end{tabular}}} 
  \\   \cline{1-1}
		\textbf{Models $\downarrow$}   &   & &   &&&   &                                                                      \\ \hline 
 
AlexNet & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & -& - \\
 \hline 

ResNet-18 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark& -\\
\hline

ResNet-50 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & - & -\\
\hline

 \hline
\end{tabular}
\end{table*}

==> header.tex <==
\usepackage[colorinlistoftodos,textsize=tiny]{todonotes}
\usepackage{multirow}
%\usepackage[colorinlistoftodos,textsize=tiny]{todonotes}
\usepackage{booktabs}
\usepackage{nicefrac}
\usepackage{amsmath,bm,dsfont,bbm,mathtools}
%\usepackage{amssymb}
\usepackage{algorithmic}
\usepackage{amsthm,nccmath,lipsum,cuted}
\usepackage{xcolor}
%\usepackage[dvips]{color}
\usepackage{colortbl}
\usepackage{graphicx}
\usepackage[lined,boxed,commentsnumbered, ruled,linesnumbered]{algorithm2e}
%\usepackage{subfigure}
\usepackage{subcaption}
\usepackage{cleveref}
%\captionsetup[subfigure]{subrefformat=simple,labelformat=simple}
\renewcommand\thesubfigure{\alph{subfigure}}
\usepackage{amsfonts}
\usepackage{ragged2e}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\usepackage{graphicx}
\usepackage{verbatim}
\usepackage{supertabular}
\usepackage{multicol}
\usepackage{physics}
\usepackage{comment}
\usepackage{dblfloatfix} 
\usepackage{bbm}
%\usepackage[footnote,draft,danish,silent,nomargin]{fixme}
\usepackage{ulem}

\newcommand{\jpcol}[1]{{\color{red} #1}}

\def\P{{\mathbb P}} 
\def\p{{p}}
\def\Q{{\bm Q}} 
\def\E{{\mathbb E}}  %%%   for "expectation value" (in math mode)
\def\ceild{{\frac{\lceil \lambda d \rceil}{\lambda}}}
%Number's sets
\def\REAL{{\mathds R}}   % Real numbers
\def\PREAL{{\mathds{R}_{\geq 0}}}   % Real numbers
\def\COMP{{\mathds C}}   % Complex numbers
\def\NAT{{\mathds N}}   % Natural numbers
\def\INTGR{{\mathds Z}}   % Integer numbers
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\def\mx{{$(\min, \times)$}}
\def\sr{{$(\sigma(s), \rho(s))$}}
\graphicspath{{./figs/}}
\usepackage[utf8]{inputenc}
 \pagenumbering{arabic}

% ------------ ARTICLE ANNOTATIONS / OTHER ------------ %

\newif\ifannote
\annotetrue  % comment this line to disable annotations

\ifannote
    \newcommand{\anninsert}[2]{{\color{#1}#2}}
    \newcommand{\anncomment}[3]{{\color{#1}[#2: #3]}}
\else
    \newcommand{\anninsert}[2]{#2}
    \newcommand{\anncomment}[3]{}
\fi

\newcommand{\jp}[1]{\anninsert{orange}{#1}}
\newcommand{\ab}[1]{\anninsert{violet}{#1}}
\newcommand{\pd}[1]{\anninsert{brown}{#1}}
\newcommand{\ia}[1]{\anninsert{red}{#1}}
\newcommand{\jg}[1]{\anninsert{cyan}{#1}}

\newcommand{\JP}[1]{\anncomment{blue}{JP}{#1}}
\newcommand{\AB}[1]{\anncomment{blue}{AB}{#1}}
\newcommand{\RM}[1]{\anncomment{blue}{RM}{#1}}
\newcommand{\PD}[1]{\anncomment{blue}{PD}{#1}}
\newcommand{\IA}[1]{\anncomment{blue}{IA}{#1}}
\newcommand{\JG}[1]{\anncomment{blue}{JG}{#1}}

\newcommand{\pkg}[1]{\texttt{#1}} 
\newcommand{\lib}[1]{\texttt{#1}}


